Lightweight, Secure and Stateful Serverless Computing with PSL

We present PSL, a lightweight, secure and stateful Function-as-a-Serivce (FaaS) framework for Trusted Execution Environments (TEEs). The framework provides rich programming language support on heterogeneous TEE hardware for statically compiled binaries and/or WebAssembly (WASM) bytecodes, with a familiar Key-Value Store (KVS) interface to secure, performant, network-embedded storage. It achieves near-native execution speeds by utilizing the dynamic memory mapping capabilities of Intel SGX2 to create an in-enclave WASM runtime with Just-In-Time (JIT) compilation. PSL is designed to efficiently operate within an asynchronous environment with a distributed tamper-proof confidential storage system, assuming minority failures. The system exchanges eventually-consistent state updates across nodes while utilizing release-consistent locking mechanisms to enhance transactional capabilities. The execution of PSL is up to 3.7x faster than the state-of-the-art SGX WASM runtime. PSL reaches 95k ops/s with YCSB 100% read workload and 89k ops/s with 50% read/write workload. We demonstrate the scalability and adaptivity of PSL through a case study of secure and distributed training of deep neural networks.

==> acks.tex <==
% \section*{Acknowledgements}

% \section*{Acknowledgement}
% This research was performed at the AUTOLAB at UC Berkeley in affiliation with the Berkeley AI Research (BAIR) Lab. The authors were supported in part by donations from  Bosch, Toyota Research Institute, Google, Siemens, and Autodesk and by equipment grants from PhotoNeo, NVidia, and Intuitive Surgical. The research is also supported by C3.ai Digital Transformation Institute for AI resilience. 


% This research was performed at the AUTOLab at UC Berkeley in affiliation with the Berkeley AI Research (BAIR) Lab, the CITRIS ``People and Robots'' (CPAR) Initiative, the Real-Time Intelligent Secure Execution (RISE) Lab, and by the NSF/VMware Partnership on Edge Computing Data Infrastructure (ECDI) Secure Fog Robotics Project Award 1838833. This research was supported in part by Bosch. 
% We thank our colleagues for helpful discussions and testing.

==> figures/consistency_time.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-0.7,xscale=1]
%uncomment if require: \path (0,646); %set diagram left start at 0, and has height of 646

%Straight Lines [id:da2686860460475995] 
\draw    (101,130) -- (615,130) ;
\draw [shift={(617,130)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da628749793806425] 
\draw    (100,180) -- (614,180) ;
\draw [shift={(616,180)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da5729498257453862] 
\draw    (100,231) -- (614,231) ;
\draw [shift={(616,231)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da35341175410306747] 
\draw    (100,281) -- (614,281) ;
\draw [shift={(616,281)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da5425720357766859] 
\draw    (100,331) -- (614,331) ;
\draw [shift={(616,331)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da06255708212690947] 
\draw    (99,381) -- (613,381) ;
\draw [shift={(615,381)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da009313535947715224] 
\draw [blue]   (120,130) -- (179.44,177.75) ;
\draw [shift={(181,179)}, rotate = 218.77] [color={rgb, 255:red, 0; green, 0; blue, 255 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da22087780752880426] 
\draw [blue]   (120,130) -- (275.32,229.92) ;
\draw [shift={(277,231)}, rotate = 212.75] [color={rgb, 255:red, 0; green, 0; blue, 255 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da08377965437017587] 
\draw[blue]    (120,130) -- (242.73,279.45) ;
\draw [shift={(244,281)}, rotate = 230.61] [color={rgb, 255:red, 0; green, 0; blue, 255 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da08046148029732691] 
\draw[dashed, red]    (120,130) -- (589.16,330.21) ;
\draw [shift={(591,331)}, rotate = 203.11] [color={rgb, 255:red, 255; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da6646494091432178] 
\draw[dashed, red]    (120,130) -- (586.24,380.05) ;
\draw [shift={(588,381)}, rotate = 208.21] [color={rgb, 255:red, 255; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da9690667053989308] 
\draw [blue]   (244,281) -- (525.24,129.95) ;
\draw [shift={(527,129)}, rotate = 151.76] [color={rgb, 255:red, 0; green, 0; blue, 255 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da7308496070942645] 
\draw [blue]   (277,231) -- (505.17,129.81) ;
\draw [shift={(507,129)}, rotate = 156.08] [color={rgb, 255:red, 0; green, 0; blue, 255 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

% Text Node
\draw (65,115) node [anchor=north west][inner sep=0.75pt]   [align=left] {\Huge $W_1$};
% Text Node
\draw (70,165) node [anchor=north west][inner sep=0.75pt]   [align=left] {\Huge $S_1$};
% Text Node
\draw (70,217) node [anchor=north west][inner sep=0.75pt]   [align=left] {\Huge $S_2$};
% Text Node
\draw (70,266) node [anchor=north west][inner sep=0.75pt]   [align=left] {\Huge $S_3$};
% Text Node
\draw (65,316) node [anchor=north west][inner sep=0.75pt]   [align=left] {\Huge $W_2$};
% Text Node
\draw (44,364) node [anchor=north west][inner sep=0.75pt]   [align=left] {\Huge $Sync$};

\end{tikzpicture}


==> figures/consistent_cut.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-0.6,xscale=0.6]
%uncomment if require: \path (0,646); %set diagram left start at 0, and has height of 646

%Shape: Rectangle [id:dp32737796475373404] 
\draw  [fill={rgb, 255:red, 254; green, 255; blue, 0 }  ,fill opacity=1 ] (111,132) -- (181,132) -- (181,172) -- (111,172) -- cycle ;
%Shape: Rectangle [id:dp44306620500171867] 
\draw  [fill={rgb, 255:red, 254; green, 255; blue, 0 }  ,fill opacity=1 ] (243,131) -- (313,131) -- (313,171) -- (243,171) -- cycle ;
%Shape: Rectangle [id:dp2656380857693532] 
\draw  [fill={rgb, 255:red, 254; green, 255; blue, 0 }  ,fill opacity=1 ] (376,130) -- (446,130) -- (446,170) -- (376,170) -- cycle ;
%Shape: Rectangle [id:dp07915274793268634] 
\draw  [fill={rgb, 255:red, 254; green, 255; blue, 0 }  ,fill opacity=1 ] (509,131) -- (579,131) -- (579,171) -- (509,171) -- cycle ;
%Left Arrow [id:dp7878910599184954] 
\draw  [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 247; green, 6; blue, 6 }  ,fill opacity=1 ] (181,149.5) -- (205.4,141) -- (205.4,145.25) -- (242,145.25) -- (242,153.75) -- (205.4,153.75) -- (205.4,158) -- cycle ;
%Left Arrow [id:dp9892886371152982] 
\draw  [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 247; green, 6; blue, 6 }  ,fill opacity=1 ] (314,149.5) -- (338.4,141) -- (338.4,145.25) -- (375,145.25) -- (375,153.75) -- (338.4,153.75) -- (338.4,158) -- cycle ;
%Left Arrow [id:dp7179498046116557] 
\draw  [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 247; green, 6; blue, 6 }  ,fill opacity=1 ] (447,148.5) -- (471.4,140) -- (471.4,144.25) -- (508,144.25) -- (508,152.75) -- (471.4,152.75) -- (471.4,157) -- cycle ;
%Shape: Rectangle [id:dp7643717629536342] 
\draw  [fill={rgb, 255:red, 254; green, 255; blue, 0 }  ,fill opacity=1 ] (112,232) -- (182,232) -- (182,272) -- (112,272) -- cycle ;
%Shape: Rectangle [id:dp3154875763351903] 
\draw  [fill={rgb, 255:red, 254; green, 255; blue, 0 }  ,fill opacity=1 ] (244,231) -- (314,231) -- (314,271) -- (244,271) -- cycle ;
%Shape: Rectangle [id:dp6376978383313403] 
\draw  [dash pattern={on 4.5pt off 4.5pt}] (377,230) -- (447,230) -- (447,270) -- (377,270) -- cycle ;
%Shape: Rectangle [id:dp851061840710208] 
\draw  [fill={rgb, 255:red, 254; green, 255; blue, 0 }  ,fill opacity=1 ] (510,231) -- (580,231) -- (580,271) -- (510,271) -- cycle ;
%Left Arrow [id:dp39008785470636176] 
\draw  [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 247; green, 6; blue, 6 }  ,fill opacity=1 ] (182,249.5) -- (206.4,241) -- (206.4,245.25) -- (243,245.25) -- (243,253.75) -- (206.4,253.75) -- (206.4,258) -- cycle ;
%Left Arrow [id:dp937170307111542] 
\draw  [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][dash pattern={on 4.5pt off 4.5pt}] (315,249.5) -- (339.4,241) -- (339.4,245.25) -- (376,245.25) -- (376,253.75) -- (339.4,253.75) -- (339.4,258) -- cycle ;
%Left Arrow [id:dp9568235244451861] 
\draw  [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 247; green, 6; blue, 6 }  ,fill opacity=1 ] (448,248.5) -- (472.4,240) -- (472.4,244.25) -- (509,244.25) -- (509,252.75) -- (472.4,252.75) -- (472.4,257) -- cycle ;
%Shape: Rectangle [id:dp3510691226276845] 
\draw  [fill={rgb, 255:red, 254; green, 255; blue, 0 }  ,fill opacity=1 ] (112,325) -- (182,325) -- (182,365) -- (112,365) -- cycle ;
%Shape: Rectangle [id:dp9324194689695904] 
\draw  [fill={rgb, 255:red, 254; green, 255; blue, 0 }  ,fill opacity=1 ] (244,324) -- (314,324) -- (314,364) -- (244,364) -- cycle ;
%Shape: Rectangle [id:dp9765725496332838] 
\draw  [dash pattern={on 4.5pt off 4.5pt}] (377,323) -- (447,323) -- (447,363) -- (377,363) -- cycle ;
%Shape: Rectangle [id:dp3499489189815157] 
\draw  [dash pattern={on 4.5pt off 4.5pt}] (510,324) -- (580,324) -- (580,364) -- (510,364) -- cycle ;
%Left Arrow [id:dp038703759431460094] 
\draw  [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 247; green, 6; blue, 6 }  ,fill opacity=1 ] (182,342.5) -- (206.4,334) -- (206.4,338.25) -- (243,338.25) -- (243,346.75) -- (206.4,346.75) -- (206.4,351) -- cycle ;
%Left Arrow [id:dp10152116860876514] 
\draw  [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][dash pattern={on 4.5pt off 4.5pt}] (315,342.5) -- (339.4,334) -- (339.4,338.25) -- (376,338.25) -- (376,346.75) -- (339.4,346.75) -- (339.4,351) -- cycle ;
%Left Arrow [id:dp7932662791686231] 
\draw  [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][dash pattern={on 4.5pt off 4.5pt}] (448,341.5) -- (472.4,333) -- (472.4,337.25) -- (509,337.25) -- (509,345.75) -- (472.4,345.75) -- (472.4,350) -- cycle ;
%Curve Lines [id:da7056711634202015] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (303.68,413.53) .. controls (317.66,410.48) and (325.12,402.39) .. (328.81,391.11) .. controls (331.23,383.72) and (332.05,374.99) .. (332.05,365.43) .. controls (332.05,354.45) and (330.96,342.39) .. (329.87,329.97) .. controls (329.33,323.87) and (328.8,317.7) .. (328.39,311.52) .. controls (327.96,305.01) and (327.68,298.5) .. (327.68,292.1) .. controls (327.68,269.4) and (331.33,247.97) .. (344.86,232.03) .. controls (361.14,212.86) and (383.24,201.57) .. (406.17,190.31) .. controls (407.46,189.68) and (408.74,189.05) .. (410.03,188.42) .. controls (412.42,187.25) and (414.81,186.07) .. (417.21,184.88) .. controls (454.04,166.57) and (490.94,145) .. (506.55,86.61)(304.32,416.47) .. controls (319.54,413.14) and (327.65,404.32) .. (331.66,392.05) .. controls (334.17,384.39) and (335.05,375.34) .. (335.05,365.43) .. controls (335.05,354.37) and (333.95,342.22) .. (332.86,329.71) .. controls (332.32,323.63) and (331.79,317.48) .. (331.39,311.32) .. controls (330.96,304.88) and (330.68,298.44) .. (330.68,292.1) .. controls (330.68,270.17) and (334.05,249.39) .. (347.14,233.97) .. controls (363.16,215.11) and (384.94,204.07) .. (407.49,193) .. controls (408.78,192.37) and (410.06,191.74) .. (411.35,191.11) .. controls (413.74,189.94) and (416.14,188.76) .. (418.54,187.57) .. controls (456.08,168.91) and (493.56,146.84) .. (509.45,87.39) ;
%Curve Lines [id:da4792662130719758] 
\draw [color={rgb, 255:red, 126; green, 211; blue, 33 }  ,draw opacity=1 ]   (350.55,423.38) .. controls (346.41,407.81) and (344.52,394.14) .. (344.52,382.14) .. controls (344.52,348.46) and (359.36,327.73) .. (381.89,314.51) .. controls (405.99,300.36) and (439.01,294.89) .. (472.05,291.38) .. controls (481.35,290.39) and (490.66,289.56) .. (499.76,288.72) .. controls (540.1,285.02) and (576.63,281.57) .. (590.84,264.05) .. controls (605.29,246.24) and (611.41,225.1) .. (611.96,203.96) .. controls (611.98,202.92) and (612,201.88) .. (612,200.83) .. controls (612,160.98) and (592.68,121.66) .. (572.06,105.17)(353.45,422.62) .. controls (349.39,407.33) and (347.52,393.92) .. (347.52,382.14) .. controls (347.52,349.77) and (361.74,329.81) .. (383.41,317.09) .. controls (407.18,303.14) and (439.78,297.82) .. (472.36,294.36) .. controls (481.65,293.38) and (490.94,292.54) .. (500.03,291.71) .. controls (541.51,287.91) and (578.63,283.86) .. (593.16,265.95) .. controls (608.05,247.59) and (614.39,225.82) .. (614.95,204.04) .. controls (614.98,202.97) and (615,201.9) .. (615,200.83) .. controls (615,159.96) and (595.06,119.72) .. (573.94,102.83) ;

% Text Node
\draw (59,137) node [anchor=north west][inner sep=0.75pt]  [font=\LARGE] [align=left] {{\LARGE $W_1$}};
% Text Node
\draw (58,234) node [anchor=north west][inner sep=0.75pt]  [font=\LARGE] [align=left] {{\LARGE $W_2$}};
% Text Node
\draw (57,330) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\LARGE $W_3$}};

\end{tikzpicture}


==> tables/cost.tex <==


\begin{table}[t]
    \centering
    \footnotesize
    \scalebox{0.9}{% Scale the table to 90% of its original size
    \begin{tabular}{lcccccc}
    \toprule
            & Server & Single Server & \multicolumn{3}{c}{\algname (USD per Hour)}\\
    Application & Core &  (USD per Hour) & On-Demand & & {Spot VM} \\
    \midrule
    YOLO & 16 & 0.40 (1.17x) & 0.80 (2.34x) & & {0.34 (1x)} \\
    SAM & 4$^*$ & 0.53 (1.21x) & 1.06 (2.42x) & & {0.44 (1x)} \\
    MPT-Home & 32 & 1.79 (1.05x) & 3.58 (2.10x) & & {1.69 (1x)} \\
    MPT-Cubicles & 32 & 1.79 (1.05x) & 3.58 (2.10x) & & {1.69 (1x)} \\
    MPT-TwistyCool & 64 & 3.58 (2.13x) & 7.16 (4.26x) & & {1.68 (1x)} \\
    Pick-Scan-Place & 16 & 0.40 (1.17x) & 0.80 (2.34x) & & {0.34 (1x)} \\
    \bottomrule
    \end{tabular}
    }
    \caption{\textbf{\algname hourly cost (USD per Hour) comparison to a Single-Server (one on-demand cloud machine)} \algname can use two on-demand machines deployment or spot VMs. In SAM, we use Nvidia T4 GPU accelerator for the inference. \algname is cheaper to run 2 spot VMs as opposed to a single server deployment up to 2.13x. }
    \label{tab:eval:cost}
\end{table}

% \begin{table}[t]
%     \centering
%     \footnotesize
%     \begin{tabular}
%         {@{}l | @{\quad}c@{\quad} | c@{\quad}  | c@{\;} c@{\quad}c@{\;}c@{\;}c@{}}\toprule
%                     & Server &Single &  \multicolumn{3}{c}\algname  \\
%          Application & Core      &Server &   On-Demand  & & {Spot VM} \\ \midrule
%          YOLO & 16  & 0.40 (1.17x) &    0.80 (2.34x)     & & {0.34 (1x)}   \\ % spot 0.17
%          SAM & 4$^*$  & 0.53 (1.21x) &    1.06 (2.42x)    & & {0.44 (1x)} \\ % spot 0.223
%          % MPT-Apartment & 16   &0.90 (1.09x)  &  1.80 (2.18x)  &{0.82 (1x)} &  \\ % spot 0.17
%          MPT-Home        & 32   &1.79 (1.05x) & 3.58 (2.10x)  & &{1.69 (1x)} \\ 
%          MPT-Cubicles & 32  &1.79 (1.05x) &   3.58 (2.10x)    & &{1.69 (1x) }  \\ 
%          MPT-TwistyCool & 64 &3.58 (2.13x) &  7.16 (4.26x)  & &{1.68 (1x)}  \\ 
%         Pick-Scan-Place & 16  & 0.40 (1.17x) &    0.80 (2.34x)     & & {0.34 (1x)}    \\ 
%          \bottomrule
%     \end{tabular}
%     \caption{\textbf{\algname hourly cost (USD per Hour) comparison to a Single-Server (one on-demand cloud machine)}  \algname can use two on-demand machines deployment or spot VMs. In SAM, we use Nvidia T4 GPU accelerator for the inference. \algname is cheaper to run 2 spot VMs as opposed to a single server deployment up to 2.13x. \jeff{unclear, is this table showing USD/hour?  If so, label it in the column headers.} \jeff{Switch to booktabs, see latex comment for URL} } % https://nhigham.com/2019/11/19/better-latex-tables-with-booktabs/
%     \label{tab:eval:cost}
% \end{table}


% % \begin{table}[t]
% %     \centering
% %     \footnotesize
% %     \begin{tabular}
% %         {@{}l | @{\quad}c@{\quad} | c@{\quad} c@{\;} c@{\quad}c@{\;}c@{\;}c@{}}\toprule
% %           & Hardware & \multicolumn{3}{c}{Cost (US\$ per Hr)} \\
% %           & Used &   Single-Server & \algname \\ \midrule
         
% %          % Dex-Net & T4 GPU & 0.53 (1.21x) & 1.04 (2.36x) & 0.44 \\ % spot 0.223

% %          \bottomrule
% %     \end{tabular}
% %     \caption{\textbf{\algname hourly cost saving compared to a Single-Server (one on-demand machine) and Fault Tolerant (FT) (two on-demand machines) deployment on Vision-based Cloud Robotics} \eric{I tend to remove this table: I think the benefit of fault tolerance is clear, and we don't show as much benefit in terms of cost. I think we can do a "one more thing" later in the physical experiment section. }  }
% %     \label{tab:eval:cost}
% % \end{table}


==> tables/exp1results.tex <==
% \begin{table}
%     \centering
%     \footnotesize
%     \begin{tabular}{l l l r r } 
% \toprule
%  & Available & Failure  & Prob. Selecting  & Failure \\ 
% & Machines  & Rate (\%)& Edge(\%) &  Reduction\\
% \midrule
% 1&E-M, E-B    & 26.67 (8/30) & - & 1x, \textbf{2.2x} \\
% 2&E-M, C-W    & 6.67 (2/30)     & 30 (9/30)   &  \textbf{4x}, 1.3x \\
% 3&E-B, C-W     & 10.00 (3/30)    &  6.67 (2/30) & \textbf{5.6x}, 1x\\ 
% 4&E-M, C-E      & 30.00 (9/30)  & 46.67 (14/30) & 1x, \textbf{1.1x} \\ 
% 5&E-B, C-E      & 53.33  (16/30)   &  3.33 (1/30)  &  \textbf{1.1x}, 0.63x \\ 
% 6&E-M, C-W, C-E       &  10.00 (3/30)  & 53.33 (16/30) & 2.7x, 1x, \textbf{3.3x} \\  
% 7&E-B, C-W, C-E       &  6.67 (2/30)  & 0 (0/30)  & \textbf{8.5x}, 1.5x, 5x \\  
% \bottomrule
% \end{tabular}
% \caption{\textbf{Evaluation of \algname in Failure Reduction} \algname selects from available baseline machines and we measure the failure rate (lower the better). \algname matches or surpasses the performance of the best individual machine, reducing the failure rate by up to 8.5 times. By selecting a machine with best latency at a given moment, it can achieve even lower failure rate than up to 1.5 times lower than that of any single machine available. \eric{please help check with the numbers, i did the calculation by hand}}
% \label{tab:eval:exp1:results}
% \vspace{-8pt}
% \end{table}

% \begin{table}
%     \centering
%     \footnotesize
%     \begin{tabular}{l l l l } 
% \toprule
%  Failure & Delay: 20 + 50ms   &  Delay: 20 + 50ms\\ 
%  Rate(\%) & 50\%   Applied     &  100\%  Applied  \\
% \midrule
% Edge1(Delay) &  26.7(8/30)  &  56.7 (17/30)        \\
%     + Edge 2 &  0.0  &  0.0       \\
%     + Cloud(West) &  10.0(3/30)  &  6.7   \\
%     + Cloud(East) &  30.0(9/30)  &  53.3   \\
%     + Cloud(East) + Cloud(West) &  6.7(2/30)   &  10.0   \\
% \bottomrule
% \end{tabular}
% \caption{\textbf{Evaluation of \algname in Failure Reduction} \algname selects from available baseline machines and we measure the failure rate (lower the better). \algname matches or surpasses the performance of the best individual machine, reducing the failure rate by up to 8.5 times. By selecting a machine with best latency at a given moment, it can achieve even lower failure rate than up to 1.5 times lower than that of any single machine available.}
% \label{tab:eval:exp1:results}
% \vspace{-8pt}
% \end{table}

\begin{table*}
    \centering
    \setlength{\tabcolsep}{10pt} 
    \renewcommand{\arraystretch}{1.5} % Default value: 1

    \footnotesize
    \begin{tabular}  {l | c | c c c c c c} 
\toprule
 % Failure Rate & Edge 1(Delay)  &  Edge 1(Delay) & Edge 1(Delay) & Edge 1(Delay) \\ 

 Edge 1 (Add Delay) & Edge 1 & Edge 1 & & & \\ 
 Failure Rate (\%)  & Only & + Edge 2     &  + Cloud(W) & + Cloud(E) & + Cloud(W) + Cloud(E)  \\
\hline
 100\% Applied &  56.7\% & 0.0\% & 10.0\% & 30.0\% & \bf{6.7\%}    \\
 % \midrule
    (Failure Reduction) &   & $(\infty)$ & (5.7x) & (1.9x) & \bf{(8.5x)}    \\
\hline
    50\% Applied &  26.7\%  & 0.0\% & \bf{6.7\%} & 53.3\% & 10.0\%  \\
% \midrule
   (Failure Reduction) &   &  ($\infty$) & \bf{(4.0x)} & (0.5x) & (2.7x)  \\
    % + Cloud(East) + Cloud(West) &  6.7(2/30)   &  10.0   \\
\bottomrule
\end{tabular}

\caption{\textbf{When local network was congested, \algname reduced failures:} Upon application of random network delays on Edge \#1, \algname automatically re-route to alternative services, i.e. Edge 2, Cloud(W), Cloud(E).  
Such automatic switching functionality to an alternative, location independent service(s) improves robustness of the system and reduced failure rate (lower the better) of the overall system. 
\algname matches performance of the best individual machine, reducing the failure rate by up to 8.5 times by selecting the best available machine compared to single edge service system under heavy network congestion.
We also showed that \algname enabled flexible yet reliable access to open cloud services via Anycast to reduce failure rate.}
\label{tab:eval:exp1:results}
\vspace{-8pt}
\end{table*}

==> tables/exp1setup.tex <==
\begin{table}
    \centering
    \footnotesize
    \begin{tabular}{ l l l | c c } 
\toprule
 & Candidates & Failure  & Interference  & Interference\\ 
  &          & Rate (\%)& (ms) & Prob. (\%)\\
\midrule
 E-G&Edge (Good)    & 0 (0/30)     & 0     & 0\\
 E-M&Edge (Medium)  & 26.67 (8/30) & $35\pm15$ & 50\\ 
 E-B&Edge (Bad)     & 56.67 (17/30)  & $35\pm15$ & 100\\ 
 C-W&Cloud (West US)     & 10  (3/30)   & -     & -\\ 
 C-E&Cloud (East US)       &  36.67 (10/30)  & -     & -\\ 
\bottomrule
\end{tabular}
\caption{\textbf{Failure Rate and Network Setups of Baseline Machines For Visual Distance Estimation}  The robot controller maintains a direct and stable connection to the Edge server via an Ethernet cable. Interference is introduced with a $35\pm15$ ms network delay, applied at rates of 50\% and 100\% to respectively represent Edge (Medium) and Edge (Bad) conditions. All the robots and edge servers are at California (West US), and the Cloud servers are located at AWS facilities in Oregon (West US) and Ohio (East US). \eric{is 35+-15 the same as 20 + 50? the latter one might be confusing} \marcus{Michael says it's just $50 \pm 0$ ms (no randomness).}
}
\label{tab:eval:exp1:setup}
\vspace{-8pt}
\end{table}

==> tables/time.tex <==

% column: application, experiment time, average uptime, total preemptions 
\begin{table}[t]
    \centering
    \footnotesize
    \begin{tabular}{@{}l@{\quad}c@{\quad} c@{\quad}c@{\quad}c@{\quad}c@{\;}c@{\;}c@{}}\toprule
           & Experiment & Preemptions & 1 Response  & 2 Response &  \\
           &  Time (hr) & Experienced & Rate (\%)  & Rate (\%)  \\
         \midrule
        
         YOLO &  25  & 2 & 100 & 75  \\
         SAM  &  25  & 3  & 100  & 75 \\ 
         Dex-Net  &  25  &  3 & 100  & 75 \\ 
         MPT  &  25  & 3  & 100  &75 \\ 
         \bottomrule
    \end{tabular}
    \caption{\textbf{\algname experiment uptime on Cloud Robotics applications} We run all cloud robotics applications with more than 24 hours period and experienced more than 2 preemptions. \algname is able to provide at least one response for all the applications despite the preemptions, and with X \% of receiving responses from multiple servers.\eric{response rate are placeholders}  }
    \label{tab:eval:time}
\end{table}

